VLT/FLAMES high-resolution chemical abundances in Sculptor: a textbook dwarf spheroidal galaxy

We present detailed chemical abundances for 99 red-giant branch stars in the centre of the Sculptor dwarf spheroidal galaxy, obtained from high-resolution VLT/FLAMES spectroscopy. This includes abundances of Li (detected in 1 out of 99 stars), Na, $\alpha$-elements (O, Mg, Si, Ca Ti), iron-peak elements (Sc, Cr, Fe, Co, Ni, Zn), r- and s-process elements (Ba, La, Nd, Eu). The sample, covering -2.3< [Fe/H]<-0.9, populates the whole metallicity distribution of the galaxy with the exception of the very low metallicity tail. There is a marked decrease in [$\alpha$/Fe] over our sample, from the Galactic halo plateau value at low [Fe/H] and then, after a `knee', a decrease to sub-solar [$\alpha$/Fe] at high [Fe/H]. This is consistent with products of core-collapse supernovae dominating at early times, followed by the onset of supernova type Ia as early as 12 Gyrs ago. The products from low-mass asymptotic giant branch stars, as traced by the s-process, also participate in the chemical evolution of Sculptor with a timescale comparable to that of supernovae type Ia. The r-process is consistent with having no time delay relative to core-collapse SN at the later stages of the chemical evolution in Sculptor. We derive empirical constraints on the relative importance of supernovae type II and Ia to the nucleosynthesis of individual iron-peak and $\alpha$-elements. The most important contribution of supernovae type Ia is to the iron-peak elements: Fe, Cr and Mn; but there is also a modest but non-negligible contribution to both the heavier $\alpha$-elements: S, Ca and Ti, and some of the iron-peak elements: Sc and Co. We see only very small or no contribution to O, Mg, Ni and Zn from supernovae type Ia in Sculptor. The observed chemical abundances in Sculptor show no evidence of a significantly different initial mass function, compared to that of the Milky Way.

==> Table_C2c.tex <==
\clearpage
\begin{deluxetable}{lrrrc|clrrr}
%\tabletypesize{\small}
\small
\tablecaption{Line list\label{table:linelist}}
\tablewidth{0pt}
\tablehead{
\colhead{Ion} &\colhead{Wavelength}  & \colhead{$\chi$}  &  \colhead{log gf}  
  & \colhead{Ref} & \colhead{~~}&\colhead{Wavelength}  & \colhead{$\chi$}  &  
\colhead{log gf}  & \colhead{Ref} \\[.2ex]
\colhead{(\AA)}    & \colhead{(eV)}   &\colhead{dex}    &\colhead{~~}  & \colhead{~~}&\colhead{~~} &\colhead{(\AA)}    & \colhead{(eV)}   &\colhead{dex}    &\colhead{~~}
}
\startdata
\\
\ion{Fe}{I} & & &                         &&& \ion{Fe}{I} (cont'd) &&&\\                        
4966.10 &  3.33 &  -0.890 &   S03 &&& 6187.99 &  3.94 &  -1.580 &   S03 \\ 
5006.12 &  2.83 &  -0.628 &   S03 &&& 6191.57 &  2.43 &  -1.416 &   S03 \\ 
5079.75 &  0.99 &  -3.240 &   S03 &&& 6213.43 &  2.22 &  -2.660 &   S03 \\ 
5083.35 &  0.96 &  -2.862 &   S03 &&& 6219.29 &  2.20 &  -2.438 &   S03 \\ 
5150.85 &  0.99 &  -3.030 &   S03 &&& 6229.23 &  2.84 &  -2.900 &   S03 \\ 
5151.92 &  1.01 &  -3.326 &   S03 &&& 6230.74 &  2.56 &  -1.276 &   S03 \\ 
5159.05 &  4.28 &  -0.810 &   S03 &&& 6240.66 &  2.22 &  -3.230 &   S03 \\ 
5162.29 &  4.18 &   0.020 &   S03 &&& 6252.57 &  2.40 &  -1.757 &   S03 \\ 
5165.41 &  4.22 &  -0.040 &   S03 &&& 6290.97 &  4.73 &  -0.760 &   S03 \\ 
5166.28 &  0.00 &  -4.200 &   S03 &&& 6297.80 &  2.22 &  -2.740 &   S03 \\ 
5171.61 &  1.48 &  -1.751 &   S03 &&& 6301.50 &  3.65 &  -0.720 &   S03 \\ 
5192.34 &  3.00 &  -0.520 &   S03 &&& 6302.49 &  3.69 &  -1.150 &   S03 \\ 
5196.08 &  4.26 &  -0.450 &   S03 &&& 6311.51 &  2.83 &  -3.220 &   S03 \\ 
5215.19 &  3.27 &  -0.930 &   S03 &&& 6355.04 &  2.84 &  -2.290 &   S03 \\ 
5216.28 &  1.61 &  -2.102 &   S03 &&& 6380.75 &  4.19 &  -1.500 &   S03 \\ 
5217.30 &  3.21 &  -1.270 &   S03 &&& 6392.54 &  2.28 &  -3.950 &   S03 \\ 
5232.95 &  2.94 &  -0.067 &   S03 &&& 6393.61 &  2.43 &  -1.630 &   S03 \\ 
5250.21 &  0.12 &  -4.700 &   S03 &&& 6419.96 &  4.73 &  -0.240 &   S03 \\ 
5253.02 &  2.28 &  -3.810 &   S03 &&& 6421.36 &  2.28 &  -2.014 &   S03 \\ 
5307.37 &  1.61 &  -2.812 &   S03 &&& 6430.86 &  2.18 &  -1.946 &   S03 \\ 
5324.19 &  3.21 &  -0.100 &   S03 &&& 6498.94 &  0.96 &  -4.690 &   S03 \\ 
5339.93 &  3.27 &  -0.680 &   S03 &&& 6518.37 &  2.83 &  -2.460 &   S03 \\ 
5364.86 &  4.45 &   0.220 &   S03 &&& 6574.23 &  0.99 &  -5.020 &   S03 \\ 
5367.48 &  4.42 &   0.550 &   S03 &&& 6581.22 &  1.48 &  -4.680 &   S03 \\ 
5369.96 &  4.37 &   0.540 &   S03 &&& 6593.88 &  2.43 &  -2.390 &   S03 \\ 
5371.50 &  0.96 &  -1.644 &   S03 &&& 6608.03 &  2.28 &  -3.940 &   S03 \\ 
5383.37 &  4.31 &   0.500 &   S03 &&& 6609.12 &  2.56 &  -2.660 &   S03 \\ 
5389.48 &  4.42 &  -0.400 &   S03 &&&   \ion{Fe}{II}  &&&\\                             
5393.17 &  3.24 &  -0.920 &   S03 &&& 4923.92 &  2.89 &  -1.320 &   S03 \\  
5397.14 &  0.91 &  -1.992 &   S03 &&& 5018.43 &  2.89 &  -1.220 &   S03 \\ 
5400.51 &  4.37 &  -0.150 &   S03 &&& 5196.08 &  4.26 &  -0.450 &   S03 \\ 
5405.79 &  0.99 &  -1.852 &   S03 &&& 5197.57 &  3.23 &  -2.100 &   S03 \\ 
5415.19 &  4.39 &   0.510 &   S03 &&& 5234.63 &  3.22 &  -2.118 &   S03 \\ 
5424.07 &  4.32 &   0.520 &   S03 &&& 5264.81 &  3.23 &  -3.210 &   S03 \\ 
5501.48 &  0.96 &  -3.050 &   S03 &&& 5276.00 &  3.20 &  -1.950 &   S03 \\ 
5506.79 &  0.99 &  -2.790 &   S03 &&& 5284.10 &  2.89 &  -3.190 &   S03 \\ 
5615.66 &  3.33 &   0.050 &   S03 &&& 5325.56 &  3.22 &  -2.600 &   S03 \\ 
5956.70 &  0.86 &  -4.570 &   S03 &&& 5425.25 &  3.20 &  -3.360 &   S03 \\ 
6003.03 &  3.88 &  -1.110 &   S03 &&& 5534.85 &  3.24 &  -2.920 &   S03 \\ 
6024.05 &  4.55 &  -0.110 &   S03 &&& 5991.38 &  3.15 &  -3.740 &   S03 \\ 
6027.06 &  4.07 &  -1.180 &   S03 &&& 6149.25 &  3.89 &  -2.720 &   S03 \\ 
6056.01 &  4.73 &  -0.450 &   S03 &&& 6238.38 &  3.89 &  -2.480 &   S03 \\ 
6078.50 &  4.79 &  -0.370 &   S03 &&& 6247.56 &  3.89 &  -2.360 &   S03 \\ 
6079.01 &  4.65 &  -0.950 &   S03 &&& 6369.46 &  2.89 &  -4.250 &   S03 \\ 
6082.72 &  2.22 &  -3.590 &   S03 &&& 6416.93 &  3.89 &  -2.790 &   S03 \\ 
6120.26 &  0.91 &  -5.940 &   S03 &&& 6432.68 &  2.89 &  -3.710 &   S03 \\ 
6136.62 &  2.45 &  -1.500 &   S03 &&& 6456.39 &  3.90 &  -2.080 &   S03 \\ 
6137.70 &  2.59 &  -1.366 &   S03 &&& 6516.08 &  2.89 &  -3.450 &   S03 \\ 
6151.62 &  2.18 &  -3.370 &   S03 &&& \ion{Li}{I} &&&\\                               
6157.75 &  4.07 &  -1.260 &   S03 &&& 6707.80 &  0.00 &   0.093 &   S03 \\ 
6165.36 &  4.14 &  -1.470 &   S03 &&&&&&\\
6173.34 &  2.22 &  -2.850 &   S03 &&&&&&\\ 
\hline \\   

                                
\ion{O}{I}  & & &                         &&&  \ion{Ti}{II}  (cont'd) &&&\\                       
6300.31 &  0.00 &  -9.750 &   S03 &&&  5154.07 &  1.57 &  -1.520 &   S03 \\ 
6363.79 &  0.02 & -10.250 &   S03 &&&  5226.55 &  1.57 &  -1.000 &   S03 \\ 
\ion{Na}{I}  & & &                         &&&  5381.01 &  1.57 &  -1.780 &   S03 \\ 
5682.65 &  2.10 &  -0.700 &   S03 &&&  5418.77 &  1.58 &  -2.110 &   S03 \\   
5688.21 &  2.10 &  -0.370 &   S03 &&&  6559.59 &  2.05 &  -2.019 &   P08 \\
5889.97 &  0.00 &   0.122 &   S03 &&& \ion{Cr}{I} &&& \\                          
6154.23 &  2.10 &  -1.560 &   S03 &&& 5206.04 &  0.94 &   0.019 &   S03 \\
6160.75 &  2.10 &  -1.260 &   S03 &&& 5409.80 &  1.03 &  -0.720 &   S03 \\
\ion{Mg}{I}  & & &                         &&& 6330.09 &  0.94 &  -2.920 &   S03 \\
5172.70 &  2.71 &  -0.390 &   S03 &&& \ion{Mn}{I} &&&\\                           
5528.41 &  4.35 &  -0.357 &   S03 &&& 5407.42 &  2.14 &  -1.743 &   S03 \\   
5711.09 &  4.35 &  -1.728 &   S03 &&& 5420.36 &  2.14 &  -1.460 &   S03 \\
\ion{Al}{I} & & &                         &&& 5432.55 &  0.00 &  -3.795 &   S03 \\
6696.03 &  3.14 &  -1.570 &   S03 &&& 5516.77 &  2.18 &  -1.847 &   S03 \\   
6698.67 &  3.14 &  -1.890 &   S03 &&& 6013.51 &  3.07 &  -0.252 &   S03 \\
\ion{Si}{I} & & &                         &&& 6021.82 &  3.08 &   0.035 &   S03 \\
5645.66 &  4.91 &  -2.140 &   S03 &&& \ion{Co}{I}  &&&\\                           
5665.60 &  4.90 &  -2.040 &   S03 &&& 5483.34 &  1.71 &  -1.488 &   S03 \\   
5684.52 &  4.93 &  -1.650 &   S03 &&& 5647.23 &  2.28 &  -1.560 &   S03 \\
6243.82 &  5.61 &  -1.270 &   S03 &&& \ion{Ni}{I} &&&\\                           
6244.48 &  5.61 &  -1.270 &   S03 &&& 5476.92 &  1.83 &  -0.890 &   S03 \\   
\ion{Ca}{I} &&&                           &&& 6176.82 &  4.09 &  -0.430 &   S03 \\
6102.73 &  1.88 &  -0.790 &   S03 &&& 6177.25 &  1.83 &  -3.500 &   S03 \\   
6122.23 &  1.89 &  -0.320 &   S03 &&& \ion{Cu}{I}  &&&\\                           
6161.30 &  2.52 &  -1.270 &   S03 &&& 5105.50 &  1.39 &  -1.505 &   S03 \\
6166.44 &  2.52 &  -1.140 &   S03 &&& 5700.24 &  1.64 &  -2.330 &   S03 \\
6169.04 &  2.52 &  -0.800 &   S03 &&& \ion{Zn}{I} &&&\\                           
6169.56 &  2.52 &  -0.480 &   S03 &&& 4810.54 &  4.08 &  -0.170 &   S03 \\
6439.08 &  2.52 &   0.390 &   S03 &&& \ion{Y}{II} &&&\\                              
6455.60 &  2.52 &  -1.290 &   S03 &&& 4883.69 &  1.08 &   0.070 &   S03 \\
6499.65 &  2.52 &  -0.820 &   S03 &&& 4900.11 &  1.03 &  -0.090 &   S03 \\
6717.68 &  2.71 &  -0.610 &   S03 &&& 5087.43 &  1.08 &  -0.170 &   S03 \\
\ion{Sc}{II} &&&                           &&& 5200.42 &  0.99 &  -0.570 &   S03 \\   
6309.90 &  1.50 &  -1.520 &   S03 &&& 5402.78 &  1.84 &  -0.510 &   L10 \\
\ion{Ti}{I} &&&                           &&& \ion{Ba}{II}  &&&\\                           
4840.87 &  0.90 &  -0.450 &   S03 &&& 5853.69 &  0.60 &  -1.010 &   S03 \\
4913.62 &  1.87 &   0.216 &   S03 &&& 6141.73 &  0.70 &  -0.077 &   S03 \\
4997.10 &  0.00 &  -2.060 &   S03 &&& 6496.91 &  0.60 &  -0.380 &   S03 \\
5016.16 &  0.85 &  -0.510 &   S03 &&& \ion{Nd}{II} &&&\\                              
5064.65 &  0.05 &  -0.930 &   S03 &&& 5249.59 &  0.98 &   0.200 &   S03 \\
5113.44 &  1.44 &  -0.727 &   S03 &&& 5319.82 &  0.55 &  -0.140 &   S03 \\
5145.47 &  1.46 &  -0.518 &   S03 &&& 5416.38 &  0.86 &  -0.980 &   L10 \\
5210.39 &  0.05 &  -0.580 &   S03 &&& 5431.54 &  1.12 &  -0.470 &   L10 \\
5978.54 &  1.87 &  -0.440 &   S03 &&& 5485.71 &  1.26 &  -0.120 &   L10 \\
5490.16 &  1.46 &  -0.933 &   S03 &&& \ion{La}{II} &&&\\                              
6126.22 &  1.07 &  -1.425 &   S03 &&& 5301.97 &  0.40 &  -1.140 &   S03 \\
6258.10 &  1.44 &  -0.355 &   P08 &&& 5303.52 &  0.32 &  -1.350 &   S03 \\
6554.24 &  1.44 &  -1.218 &   S03 &&& 6390.46 &  0.32 &  -1.400 &   S03 \\
6556.08 &  1.46 &  -1.074 &   S03 &&& 6320.43 &  0.17 &  -1.562 &   P08 \\
6743.13 &  0.90 &  -1.630 &   S03 &&& 6774.27 &  0.13 &  -1.708 &   ...  \\
\ion{Ti}{II}  &&&                           &&& \ion{Eu}{II} &&&\\                         
4798.53 &  1.08 &  -2.670 &   S03 &&& 6645.13 &  1.37 &   0.200 &   S03 \\
5129.16 &  1.89 &  -1.390 &   S03 &&& &&&
\enddata
\tablerefs{S03=Shetrone et al. (2003); P08=Pompeia et al. (2008); L10=Letarte et al. (2010)}
\end{deluxetable}

